Large language models in 6G security: challenges and opportunities

The rapid integration of Generative AI (GenAI) and Large Language Models (LLMs) in sectors such as education and healthcare have marked a significant advancement in technology. However, this growth has also led to a largely unexplored aspect: their security vulnerabilities. As the ecosystem that includes both offline and online models, various tools, browser plugins, and third-party applications continues to expand, it significantly widens the attack surface, thereby escalating the potential for security breaches. These expansions in the 6G and beyond landscape provide new avenues for adversaries to manipulate LLMs for malicious purposes. We focus on the security aspects of LLMs from the viewpoint of potential adversaries. We aim to dissect their objectives and methodologies, providing an in-depth analysis of known security weaknesses. This will include the development of a comprehensive threat taxonomy, categorizing various adversary behaviors. Also, our research will concentrate on how LLMs can be integrated into cybersecurity efforts by defense teams, also known as blue teams. We will explore the potential synergy between LLMs and blockchain technology, and how this combination could lead to the development of next-generation, fully autonomous security solutions. This approach aims to establish a unified cybersecurity strategy across the entire computing continuum, enhancing overall digital security infrastructure.

==> uml <==
@startuml
actor Red_Teamer #red

box "Attack Surface" #Pink
    participant "PenTesting Agent" as pentester
    entity "6G Infrastructure" as infra
end box

box "Initial Detection and Analysis" #LightYellow
    participant "Traffic Parser Agent" as parser
    participant "Analyzer Agent" as analyzer
end box

box "Response Generation and Execution" #LightGreen
    participant "Coder Agent" as coder
    participant "Function Caller Agent" as functionCaller
    participant "API Caller Agent" as apiCaller
    participant "RAG Agent" as rag
end box

box "Decision Support and Communication" #LightBlue
 	participant "XAI" as xai
    database "SIEM System" as siem
    participant "SIEM Assistant" as assistant
end box

Red_Teamer ->  pentester: choreographs attack
pentester -> infra : Initiates Attack
parser ->infra: request traffic data
infra --> parser : send traffic data
parser -> analyzer : sends traffic data
analyzer -> xai: requests alignment and Explainability 
xai -->analyzer: allows
analyzer -> coder : sends pcaps
coder -> functionCaller : Data enrichment
functionCaller -->coder: returns enrichmed data
coder -> apiCaller : Data enrichment
apiCaller -->coder: returns enrichmed data
coder -> rag : Requests Contextual\n Info
rag -> siem : Gathers Insights
siem -> rag : Returns Insights
rag -> coder : Provides enrichment\nAnalysis

coder -> analyzer : sends code\n for analytics
analyzer ->siem: Logs Defense Actions
siem ->coder: requests defence actions
coder -> infra: carries out response measures
infra --> pentester : returns loot/data
pentester -->Red_Teamer: reports results

actor Blue_Teamer #blue
Blue_Teamer -> assistant : Initiates chats
assistant ->siem
assistant ->xai
xai-> assistant
assistant ->Blue_Teamer: Analyzes Post-Attack\n Data
@enduml
